BULKHEAD: Secure, Scalable, and Efficient Kernel Compartmentalization with PKS

The endless stream of vulnerabilities urgently calls for principled mitigation to confine the effect of exploitation. However, the monolithic architecture of commodity OS kernels, like the Linux kernel, allows an attacker to compromise the entire system by exploiting a vulnerability in any kernel component. Kernel compartmentalization is a promising approach that follows the least-privilege principle. However, existing mechanisms struggle with the trade-off on security, scalability, and performance, given the challenges stemming from mutual untrustworthiness among numerous and complex components. In this paper, we present BULKHEAD, a secure, scalable, and efficient kernel compartmentalization technique that offers bi-directional isolation for unlimited compartments. It leverages Intel's new hardware feature PKS to isolate data and code into mutually untrusted compartments and benefits from its fast compartment switching. With untrust in mind, BULKHEAD introduces a lightweight in-kernel monitor that enforces multiple important security invariants, including data integrity, execute-only memory, and compartment interface integrity. In addition, it provides a locality-aware two-level scheme that scales to unlimited compartments. We implement a prototype system on Linux v6.1 to compartmentalize loadable kernel modules (LKMs). Extensive evaluation confirms the effectiveness of our approach. As the system-wide impacts, BULKHEAD incurs an average performance overhead of 2.44% for real-world applications with 160 compartmentalized LKMs. While focusing on a specific compartment, ApacheBench tests on ipv6 show an overhead of less than 2%. Moreover, the performance is almost unaffected by the number of compartments, which makes it highly scalable.

==> Makefile <==
MAIN ?= p
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
ODGS := $(patsubst %.odg,%.pdf,$(wildcard fig/*.odg))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(ODGS) $(PLOT)
LTEX := --latex-args="-synctex=1 -shell-escape"
BTEX := --bibtex-args="-min-crossrefs=99"
SHELL:= $(shell echo $$SHELL)

UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Darwin)
  INKSCAPE=/Applications/Inkscape.app/Contents/MacOS/inkscape
  SOFFICE=/Applications/LibreOffice.app/Contents/MacOS/soffice
else
  INKSCAPE=inkscape
  SOFFICE=soffice
endif

all: $(DEPS) ## generate a pdf
	chmod a+x bin/*
	@TEXINPUTS="sty:" bin/latexrun.py $(LTEX) $(BTEX) $(MAIN)
	cp latex.out/$(MAIN).synctex.gz .

submit: $(DEPS) ## proposal function
	@for f in $(wildcard submit-*.tex); do \
		TEXINPUTS="sty:" bin/latexrun.py $$f; \
	done

diff: $(DEPS) ## generate diff-highlighed pdf
	@bin/diff.sh $(DIFF)

help: ## print help
	@grep -E '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
	  | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-10s\033[0m %s\n", $$1, $$2}'

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
	   "$(shell git rev-parse --short HEAD)"            \
	   "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/% ## build highlighted tex code from source code
	pygmentize -P tabsize=4 -P mathescape -f latex $^ | bin/mark.py > $@

code/fmt.tex: ## generate color table
	pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg ## generate pdf from svg
	$(INKSCAPE) -D --export-type=pdf ${CURDIR}/$^ ${CURDIR}/$@

fig/%.pdf: fig/%.odg ## generate pdf from LibreOffice Draw
	$(SOFFICE) --convert-to pdf $< --outdir $(@D)
	pdfcrop $@ $@

data/%.tex: data/%.gp ## generate plot
	gnuplot $^

draft: $(DEPS) ## generate pdf with a draft info
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun.py $(BTEX) $(MAIN)

watermark: $(DEPS) ## generate pdf with a watermark
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun.py $(BTEX) $(MAIN)

spell: ## run a spell check
	@for i in *.tex fig/*.tex; do bin/aspell.sh tex $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex
	@pdftotext $(MAIN).pdf /dev/stdout | grep '??'
	@for i in fig/*.svg; do bin/aspell.sh svg $$i; done
	@for i in code/*.c; do bin/aspell.sh code $$i; done

bib: all ## print bib used in the paper
	bibexport latex.out/$(MAIN).aux

clean: ## clean up
	@bin/latexrun.py --clean
	rm -f abstract.txt
	rm -f $(MAIN).synctex.gz

distclean: clean ## clean up completely
	rm -f code/*.tex
	rm -rf _minted_p

abstract.txt: abstract.tex $(MAIN).tex ## generate abstract.txt
	@bin/mkabstract.py $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init bib


==> README <==
die: a paper template
=====================

## start

0. Prerequisites

  - Python 3.x
  - pygmentize

    $ pip install Pygments 

1. clone the git repo:

  - if you have none,

    $ git clone --depth=1 git@github.com:tsgates/die.git

  - if you have a git-repo to work on,

    $ git subtree add --squash git@github.com:tsgates/die.git master -P paper

  - or

    $ wget https://github.com/tsgates/die/releases/download/latest/die.tar.gz

2. build it:

    $ make
    p.pdf built @Tue May 20 20:38:19 EDT 2014
    
    (check p.pdf)

3. starting point, p.tex:

    $ grep -oP 'input{\K\w+' p.tex
    cmds
    rev
   *hdr
    abstract
   *ex
    intro
    overview
    design
    impl
    eval
    conclusion
    ack

  - hdr: includes title/author info
  - ex : includes latex examples

4. example latex

    $ git checkout example
    $ make

5. formatting rules (dependencies)

  - code/*.{c,cc,py,js ...} -> code/*.tex
  - fig/*.svg               -> fig/*.pdf
  - data/*.gp               -> fig/*.tex

  (see ex.tex for more details)

## tools

1. make a draft for revision

    $ make draft
    $ make watermark

2. abstract.txt (from abstract.tex)

    $ cat abstract.txt 

3. highlight changes, since the last submit

    $ make diff DIFF=HEAD@{}

4. spell check

    $ make spell

## Acknowledgment

This template contains a few files copied/stolen from the Internet and
mainly from my past collaborators (e.g., sty/*, conf.bib, some bin/),
which I couldn't keep track of their licenses.

==> code/address.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define PCI\PYZus{}VENDOR\PYZus{}ID       0x00    }\PY{c+cm}{/* 16 bits */}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define PCI\PYZus{}DEVICE\PYZus{}ID       0x02    }\PY{c+cm}{/* 16 bits */}
\PY{k}{if} \PY{p}{(}\PY{n}{pci\PYZus{}bus\PYZus{}read\PYZus{}config\PYZus{}dword}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{n}{PCI\PYZus{}VENDOR\PYZus{}ID}\PY{p}{,} \PY{n}{l}\PY{p}{)}\PY{p}{)}
    \PY{k}{return} \PY{n+nb}{false}\PY{p}{;}
\PY{n}{pci\PYZus{}read\PYZus{}config\PYZus{}word}\PY{p}{(}\PY{n}{pdev}\PY{p}{,} \PY{n}{PCI\PYZus{}DEVICE\PYZus{}ID}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{device\PYZus{}id}\PY{p}{)}\PY{p}{;}
\end{Verbatim}


==> code/fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/invaildret.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{pci\PYZus{}bus\PYZus{}read\PYZus{}dev\PYZus{}vendor\PYZus{}id}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{l}\PY{p}{,} \PY{l+m+mi}{60}\PY{o}{*}\PY{l+m+mi}{1000}\PY{p}{)}\PY{p}{)}
    \PY{k}{return} \PY{n+nb}{NULL}\PY{p}{;}

\PY{k}{if} \PY{p}{(}\PY{n}{pci\PYZus{}read\PYZus{}config\PYZus{}byte}\PY{p}{(}\PY{n}{dev}\PY{p}{,} \PY{n}{PCI\PYZus{}HEADER\PYZus{}TYPE}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{hdr\PYZus{}type}\PY{p}{)}\PY{p}{)}
    \PY{k}{return} \PY{o}{\PYZhy{}}\PY{n}{EIO}\PY{p}{;}
\end{Verbatim}


==> code/offset.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{pci\PYZus{}read\PYZus{}config\PYZus{}byte}\PY{p}{(}\PY{n}{dev}\PY{p}{,} \PY{n}{PCI\PYZus{}HEADER\PYZus{}TYPE}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{hdr\PYZus{}type}\PY{p}{)}
\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{hdr\PYZus{}type} \PY{o}{=} \PY{n}{hdr\PYZus{}type} \PY{o}{\PYZam{}} \PY{l+m+mh}{0x7f}\PY{p}{;}
\PY{n}{pci\PYZus{}bus\PYZus{}read\PYZus{}dev\PYZus{}vendor\PYZus{}id}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{l}\PY{p}{,} \PY{l+m+mi}{60}\PY{o}{*}\PY{l+m+mi}{1000}\PY{p}{)}
\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{vendor} \PY{o}{=} \PY{n}{l} \PY{o}{\PYZam{}} \PY{l+m+mh}{0xffff}\PY{p}{;}
\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{device} \PY{o}{=} \PY{p}{(}\PY{n}{l} \PY{o}{\PYZgt{}}\PY{o}{\PYZgt{}} \PY{l+m+mi}{16}\PY{p}{)} \PY{o}{\PYZam{}} \PY{l+m+mh}{0xffff}\PY{p}{;}
\PY{k}{if} \PY{p}{(}\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{vendor} \PY{o}{!}\PY{o}{=} \PY{n}{PCI\PYZus{}VENDOR\PYZus{}ID\PYZus{}INTEL}\PY{p}{)}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{.}
\end{Verbatim}


==> code/pcidevadd.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define PCI\PYZus{}CONF1\PYZus{}ADDRESS(bus, devfn, reg) \PYZbs{}}
\PY{c+cp}{    (0x80000000 | ((reg \PYZam{} 0xF00) \PYZlt{}\PYZlt{} 16) | (bus \PYZlt{}\PYZlt{} 16) \PYZbs{}}
\PY{c+cp}{    | (devfn \PYZlt{}\PYZlt{} 8) | (reg \PYZam{} 0xFC))}
\PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{n}{outl}\PY{p}{(}\PY{n}{PCI\PYZus{}CONF1\PYZus{}ADDRESS}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{n}{reg}\PY{p}{)}\PY{p}{,} \PY{l+m+mh}{0xCF8}\PY{p}{)}\PY{p}{;}
\end{Verbatim}


==> code/pciexample.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define PCI\PYZus{}VENDOR\PYZus{}ID       0x00    }\PY{c+cm}{/* 16 bits */}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define PCI\PYZus{}DEVICE\PYZus{}ID       0x02}
\PY{k}{struct} \PY{n}{bus\PYZus{}type} \PY{n}{pci\PYZus{}bus\PYZus{}type} \PY{o}{=} \PY{p}{\PYZob{}}
    \PY{p}{.}\PY{n}{probe}      \PY{o}{=} \PY{n}{pci\PYZus{}device\PYZus{}probe}\PY{p}{,}
\PY{p}{\PYZcb{}}\PY{p}{;}
\PY{k}{struct} \PY{n}{pci\PYZus{}driver} \PY{n}{e1000\PYZus{}driver} \PY{o}{=} \PY{p}{\PYZob{}}
    \PY{p}{.}\PY{n}{id\PYZus{}table} \PY{o}{=} \PY{n}{e1000\PYZus{}pci\PYZus{}tbl}\PY{p}{,}
    \PY{p}{.}\PY{n}{probe}    \PY{o}{=} \PY{n}{e1000\PYZus{}probe}\PY{p}{,}
\PY{p}{\PYZcb{}}\PY{p}{;}
\PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n+nf}{presdue\PYZus{}entry}\PY{p}{(}\PY{k}{struct} \PY{n}{pci\PYZus{}bus} \PY{o}{*}\PY{n}{bus}\PY{p}{,} \PY{k+kt}{int} \PY{n}{devfn}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{struct} \PY{n}{pci\PYZus{}dev} \PY{n}{dev} \PY{o}{=} \PY{n}{pci\PYZus{}scan\PYZus{}device}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{dev}\PY{p}{)} \PY{k}{return} \PY{n+nb}{NULL}\PY{p}{;}
\PY{p}{\PYZcb{}}
\PY{k}{struct} \PY{n}{pci\PYZus{}dev} \PY{o}{*}\PY{n+nf}{pci\PYZus{}scan\PYZus{}device}\PY{p}{(}\PY{k}{struct} \PY{n}{pci\PYZus{}bus} \PY{o}{*}\PY{n}{bus}\PY{p}{,} \PY{k+kt}{int} \PY{n}{devfn}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{n}{u32} \PY{n}{l}\PY{p}{;}
    \PY{n}{pci\PYZus{}bus\PYZus{}read\PYZus{}config\PYZus{}dword}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{n}{PCI\PYZus{}VENDOR\PYZus{}ID}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{l}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{o}{*}\PY{n}{l} \PY{o}{=}\PY{o}{=} \PY{l+m+mh}{0xffffffff} \PY{o}{|}\PY{o}{|} \PY{o}{*}\PY{n}{l} \PY{o}{=}\PY{o}{=} \PY{l+m+mh}{0x00000000}\PY{p}{)} \PY{k}{return} \PY{n+nb}{NULL}\PY{p}{;}
    \PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{vendor} \PY{o}{=} \PY{n}{l} \PY{o}{\PYZam{}} \PY{l+m+mh}{0xffff}\PY{p}{;}
    \PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{device} \PY{o}{=} \PY{p}{(}\PY{n}{l} \PY{o}{\PYZgt{}}\PY{o}{\PYZgt{}} \PY{l+m+mi}{16}\PY{p}{)} \PY{o}{\PYZam{}} \PY{l+m+mh}{0xffff}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{pci\PYZus{}read\PYZus{}config\PYZus{}byte}\PY{p}{(}\PY{n}{dev}\PY{p}{,} \PY{n}{PCI\PYZus{}HEADER\PYZus{}TYPE}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{hdr\PYZus{}type}\PY{p}{)}\PY{p}{)}
        \PY{k}{return} \PY{o}{\PYZhy{}}\PY{n}{EIO}\PY{p}{;}
\PY{p}{\PYZcb{}}
\PY{k}{struct} \PY{n}{pci\PYZus{}device\PYZus{}id} \PY{o}{*}
\PY{n+nf}{pci\PYZus{}match\PYZus{}device}\PY{p}{(}\PY{k}{struct} \PY{n}{pci\PYZus{}device\PYZus{}id} \PY{o}{*}\PY{n}{id}\PY{p}{,} \PY{k}{struct} \PY{n}{pci\PYZus{}dev} \PY{o}{*}\PY{n}{dev}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{if}\PY{p}{(}\PY{p}{(}\PY{n}{id}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{vendor}\PY{o}{=}\PY{o}{=}\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{vendor}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{n}{id}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{device}\PY{o}{=}\PY{o}{=}\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{device}\PY{p}{)}\PY{p}{)}
        \PY{k}{return} \PY{n}{id}\PY{p}{;}
    \PY{k}{return} \PY{n+nb}{NULL}\PY{p}{;}
\PY{p}{\PYZcb{}}
\PY{k+kt}{int} \PY{n+nf}{pci\PYZus{}device\PYZus{}probe}\PY{p}{(}\PY{k}{struct} \PY{n}{device} \PY{o}{*}\PY{n}{dev}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{struct} \PY{n}{pci\PYZus{}driver} \PY{o}{*}\PY{n}{drv} \PY{o}{=} \PY{n}{to\PYZus{}pci\PYZus{}driver}\PY{p}{(}\PY{n}{dev}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{driver}\PY{p}{)}\PY{p}{;}
    \PY{c+cm}{/*vendor\PYZus{}id, device\PYZus{}id are in  e1000\PYZus{}pci\PYZus{}tbl*/}
    \PY{n}{id} \PY{o}{=} \PY{n}{pci\PYZus{}match\PYZus{}device}\PY{p}{(}\PY{n}{drv}\PY{p}{,} \PY{n}{pci\PYZus{}dev}\PY{p}{)}\PY{p}{;}
    \PY{k+kt}{int} \PY{n}{rc} \PY{o}{=} \PY{n}{e1000\PYZus{}probe}\PY{p}{(}\PY{n}{dev}\PY{p}{,} \PY{n}{id}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{rc}\PY{p}{)} \PY{k}{return} \PY{n}{rc}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/pciscan.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{for} \PY{p}{(}\PY{n}{devfn} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;} \PY{n}{devfn} \PY{o}{\PYZlt{}} \PY{l+m+mh}{0x100}\PY{p}{;} \PY{n}{devfn} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{8}\PY{p}{)}
    \PY{n}{pci\PYZus{}scan\PYZus{}slot}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{)}\PY{p}{;}
\end{Verbatim}


==> fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> invaildret.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{pci\PYZus{}bus\PYZus{}read\PYZus{}dev\PYZus{}vendor\PYZus{}id}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{l}\PY{p}{,} \PY{l+m+mi}{60}\PY{o}{*}\PY{l+m+mi}{1000}\PY{p}{)}\PY{p}{)}
    \PY{k}{return} \PY{n+nb}{NULL}\PY{p}{;}

\PY{k}{if} \PY{p}{(}\PY{n}{pci\PYZus{}read\PYZus{}config\PYZus{}byte}\PY{p}{(}\PY{n}{dev}\PY{p}{,} \PY{n}{PCI\PYZus{}HEADER\PYZus{}TYPE}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{hdr\PYZus{}type}\PY{p}{)}\PY{p}{)}
    \PY{k}{return} \PY{o}{\PYZhy{}}\PY{n}{EIO}\PY{p}{;}
\end{Verbatim}


==> pcidevadd.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define PCI\PYZus{}CONF1\PYZus{}ADDRESS(bus, devfn, reg) \PYZbs{}}
\PY{c+cp}{    (0x80000000 | ((reg \PYZam{} 0xF00) \PYZlt{}\PYZlt{} 16) | (bus \PYZlt{}\PYZlt{} 16) \PYZbs{}}
\PY{c+cp}{    | (devfn \PYZlt{}\PYZlt{} 8) | (reg \PYZam{} 0xFC))}
\PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{n}{outl}\PY{p}{(}\PY{n}{PCI\PYZus{}CONF1\PYZus{}ADDRESS}\PY{p}{(}\PY{n}{bus}\PY{p}{,} \PY{n}{devfn}\PY{p}{,} \PY{n}{reg}\PY{p}{)}\PY{p}{,} \PY{l+m+mh}{0xCF8}\PY{p}{)}\PY{p}{;}
\end{Verbatim}


==> rev.tex <==
\gdef\therev{611f9db}
\gdef\thedate{2023-04-18 12:58:23 +0000}


==> sections/reference.tex <==
\begin{thebibliography}{00}
\bibitem{b1} HonggFuzz. https://github.com/google/honggfuzz
\bibitem{b2} Chen, Hongxu, et al. "Hawkeye: Towards a desired directed grey-box fuzzer." Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications Security. 2018.
\bibitem{b3} Böhme, Marcel, et al. "Directed greybox fuzzing." Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security. 2017.
\bibitem{b4} Peach Fuzzer. https://peachtech.gitlab.io/peach-fuzzer-community/
\bibitem{b5} Liang, Hongliang, et al. "Sequence coverage directed greybox fuzzing." 2019 IEEE/ACM 27th International Conference on Program Comprehension (ICPC). IEEE Computer Society, 2019.
\bibitem{b6} Kim, Juhwan, and Joobeom Yun. "Poster: Directed hybrid fuzzing on binary code." Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security. 2019.
\bibitem{b7} Du, Xiaoning, et al. "Leopard: Identifying vulnerable code for vulnerability assessment through program metrics." 2019 IEEE/ACM 41st International Conference on Software Engineering (ICSE). IEEE, 2019.
\bibitem{b8} Li, Yuwei, et al. "V-fuzz: Vulnerability-oriented evolutionary fuzzing." arXiv preprint arXiv:1901.01142 (2019).
\bibitem{b9} Liang, Hongliang, et al. "Sequence directed hybrid fuzzing." 2020 IEEE 27th International Conference on Software Analysis, Evolution and Reengineering (SANER). IEEE, 2020.
\bibitem{b10} Wüstholz, Valentin, and Maria Christakis. "Targeted greybox fuzzing with static lookahead analysis." Proceedings of the ACM/IEEE 42nd International Conference on Software Engineering. 2020.
\bibitem{b11} Österlund, Sebastian, et al. "Parmesan: Sanitizer-guided greybox fuzzing." Proceedings of the 29th USENIX Conference on Security Symposium. 2020.
\bibitem{b12} Nguyen, Manh-Dung, et al. "Binary-level Directed Fuzzing for Use-After-Free Vulnerabilities." RAID. 2020.
\bibitem{b13} Wang, Zi, Ben Liblit, and Thomas Reps. "TOFU: Target-oriented fuzzer." arXiv preprint arXiv:2004.14375 (2020).
\bibitem{b14} Wang, Pengfei, et al. "Sok: The progress, challenges, and perspectives of directed greybox fuzzing." Challenges, and Perspectives of Directed Greybox Fuzzing (2020).
\bibitem{b15} Li, Rundong, et al. "GTFuzz: Guard token directed grey-box fuzzing." 2020 IEEE 25th Pacific Rim International Symposium on Dependable Computing (PRDC). IEEE, 2020.
\bibitem{b16} Zhu, Xiaogang, et al. "Defuzz: Deep learning guided directed fuzzing." arXiv preprint arXiv:2010.12149 (2020).
\bibitem{b17} Zhu, Kailong, et al. "Constructing more complete control flow graphs utilizing directed gray-box fuzzing." Applied Sciences 11.3 (2021): 1351.
\bibitem{b18} Canakci, Sadullah, et al. "Directfuzz: Automated test generation for rtl designs using directed graybox fuzzing." 2021 58th ACM/IEEE Design Automation Conference (DAC). IEEE, 2021.
\bibitem{b19} Zhu, Xiaogang, and Marcel Böhme. "Regression greybox fuzzing." Proceedings of the 2021 ACM SIGSAC Conference on Computer and Communications Security. 2021.
\bibitem{b20} Wang, Shen, et al. "Kcfuzz: Directed fuzzing based on keypoint coverage." Artificial Intelligence and Security: 7th International Conference, ICAIS 2021, Dublin, Ireland, July 19–23, 2021, Proceedings, Part I 7. Springer International Publishing, 2021.
\bibitem{b21} Pham, Van-Thuan, et al. "Towards systematic and dynamic task allocation for collaborative parallel fuzzing." 2021 36th IEEE/ACM International Conference on Automated Software Engineering (ASE). IEEE, 2021.
\bibitem{b22} Meng, Ruijie, et al. "Finding Counterexamples of Temporal Logic Properties in Software Implementations via Greybox Fuzzing." International Conference on Software Engineering. 2022.
\bibitem{b23} Huang, Heqing, et al. "Beacon: Directed grey-box fuzzing with provable path pruning." 2022 IEEE Symposium on Security and Privacy (SP). IEEE, 2022.
\bibitem{b24} Du, Zhengjie, et al. "WindRanger: a directed greybox fuzzer driven by deviation basic blocks." Proceedings of the 44th International Conference on Software Engineering. 2022.
\bibitem{b25} Canakci, Sadullah, et al. "TargetFuzz: Using DARTs to Guide Directed Greybox Fuzzers." Proceedings of the 2022 ACM on Asia Conference on Computer and Communications Security. 2022.
\bibitem{b26} Zhang, Lei, et al. "Exploit the Last Straw That Breaks Android Systems." 2022 IEEE Symposium on Security and Privacy (SP). IEEE, 2022.
\bibitem{b27} Meng, Ruijie, et al. "Linear-time temporal logic guided greybox fuzzing." Proceedings of the 44th International Conference on Software Engineering. 2022.
\bibitem{b28} Canakci, Sadullah. Directing greybox fuzzing to discover bugs in hardware and software. Diss. Boston University, 2022.
\bibitem{b29} Liang, Hongliang, et al. "Multiple Targets Directed Greybox Fuzzing." arXiv preprint arXiv:2206.14977 (2022).
\bibitem{b30} Zong, Peiyuan, et al. "Fuzzguard: Filtering out unreachable inputs in directed grey-box fuzzing through deep learning." Proceedings of the 29th USENIX Conference on Security Symposium. 2020.
\bibitem{b31} Lee, Gwangmu, Woochul Shim, and Byoungyoung Lee. "Constraint-guided Directed Greybox Fuzzing." USENIX Security Symposium. 2021.
\bibitem{b32} American Fuzzing Loop. https://github.com/google/AFL
\bibitem{b33} LibFuzzer. https://llvm.org/docs/LibFuzzer.html
\bibitem{b34} Lu, Kangjie, and Hong Hu. "Where does it go? refining indirect-call targets with multi-layer type analysis." Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security. 2019.
\bibitem{b35} Dominator in Graph Theory, 
https://en.wikipedia.org/wiki/Dominator\_ (graph\_theory), 2019
\bibitem{b36} Liang, Hongliang, et al. "Sequence coverage directed greybox fuzzing." 2019 IEEE/ACM 27th International Conference on Program Comprehension (ICPC). IEEE Computer Society, 2019.
\bibitem{b37} Wu, Zejun, et al. "RDGFuzz: A directed greybox fuzzing optimization method based on Rich-Branch nodes." Proceedings of the 2022 6th International Conference on Electronic Information Technology and Computer Engineering. 2022.
\bibitem{b38} Zhao, Yuyue, et al. "Suzzer: A vulnerability-guided fuzzer based on deep learning." International Conference on Information Security and Cryptology. Springer, Cham, 2020.
\bibitem{b39} He, Ziheng, et al. "SwitchFuzz: Switch Short-Term Goals in Directed Grey-Box Fuzzing." Applied Sciences 12.21 (2022): 11097.
\bibitem{b40} Du, Zhengjie, et al. "WindRanger: a directed greybox fuzzer driven by deviation basic blocks." Proceedings of the 44th International Conference on Software Engineering. 2022.
\bibitem{b41} Liang, Hongliang, et al. "Sequence directed hybrid fuzzing." 2020 IEEE 27th International Conference on Software Analysis, Evolution and Reengineering (SANER). IEEE, 2020.
\bibitem{b42} Luo, Changhua, Wei Meng, and Penghui Li. "SelectFuzz: Efficient Directed Fuzzing with Selective Path Exploration." 2023 IEEE Symposium on Security and Privacy (SP). IEEE Computer Society, 2022.
\bibitem{b43} She, Dongdong, et al. "Neuzz: Efficient fuzzing with neural program smoothing." 2019 IEEE Symposium on Security and Privacy (SP). IEEE, 2019.
\bibitem{b44} Fioraldi, Andrea, et al. "AFL++ combining incremental steps of fuzzing research." Proceedings of the 14th USENIX Conference on Offensive Technologies. 2020.
\bibitem{b45} Wang, Jinghan, Chengyu Song, and Heng Yin. "Reinforcement learning-based hierarchical seed scheduling for greybox fuzzing." (2021).
\bibitem{b46} Zhang, Zhuo, et al. "Stochfuzz: Sound and cost-effective fuzzing of stripped binaries by incremental and stochastic rewriting." 2021 IEEE Symposium on Security and Privacy (SP). IEEE, 2021.
\bibitem{b47} Lughofer, Edwin, and Erich-Peter Klement. "FLEXFIS: A variant for incremental learning of Takagi-Sugeno fuzzy systems." The 14th IEEE International Conference on Fuzzy Systems, 2005. FUZZ'05.. IEEE, 2005.
\bibitem{b48} Godefroid, Patrice, Hila Peleg, and Rishabh Singh. "Learn\&fuzz: Machine learning for input fuzzing." 2017 32nd IEEE/ACM International Conference on Automated Software Engineering (ASE). IEEE, 2017.
\bibitem{b49} Chen, Peng, and Hao Chen. "Angora: Efficient fuzzing by principled search." 2018 IEEE Symposium on Security and Privacy (SP). IEEE, 2018.
\bibitem{b50} M. Soam and S. Thakur, "Next Word Prediction Using Deep Learning: A Comparative Study," 2022 12th International Conference on Cloud Computing, Data Science \& Engineering (Confluence), Noida, India, 2022, pp. 653-658, doi: 10.1109/Confluence52989.2022.9734151.
\bibitem{b51} Liu, Xiao, et al. "Deepfuzz: Automatic generation of syntax valid c programs for fuzz testing." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 33. No. 01. 2019.
\bibitem{b52} Ram, Anant, et al. "A density based algorithm for discovering density varied clusters in large spatial databases." International Journal of Computer Applications 3.6 (2010): 1-4.
\bibitem{b53} Google. Fuzzer Test Suite. https://github.com/google/fuzzer-test-suite
%\bibitem{b54} Du, Zhengjie, et al. "WindRanger: a directed greybox fuzzer driven by deviation basic blocks." Proceedings of the 44th International Conference on Software Engineering. 2022.
\bibitem{b55} P-value. https://en.wikipedia.org/wiki/P-value
\bibitem{b56} Vargha, András, and Harold D. Delaney. "A critique and improvement of the CL common language effect size statistics of McGraw and Wong." Journal of Educational and Behavioral Statistics 25.2 (2000): 101-132.
\bibitem{b57} U.S. Census Bureau. “Statistical Quality Standard E1: Analyzing Data.”
\bibitem{b58} Hazewinkel, Michiel. "Quadratic deviation." Encyclopedia of Mathematics (2001).
\bibitem{b59} Böhme, Marcel, Van-Thuan Pham, and Abhik Roychoudhury. "Coverage-based greybox fuzzing as markov chain." Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security. 2016.
\bibitem{b60} Sundermeyer, Martin, Ralf Schlüter, and Hermann Ney. "LSTM neural networks for language modeling." Thirteenth annual conference of the international speech communication association. 2012.
%\bibitem{b61} Huang, Heqing, et al. "Beacon: Directed grey-box fuzzing with provable path pruning." 2022 IEEE Symposium on Security and Privacy (SP). IEEE, 2022.
\bibitem{b62} Church, Kenneth Ward. "Word2Vec." Natural Language Engineering 23.1 (2017): 155-162.
\end{thebibliography}
\vspace{12pt}

